On Policy Reuse: An Expressive Language for Representing and Executing General Policies that Call Other Policies

Recently, a simple but powerful language for expressing and learning general policies and problem decompositions (sketches) has been introduced in terms of rules defined over a set of Boolean and numerical features. In this work, we consider three extensions of this language aimed at making policies and sketches more flexible and reusable: internal memory states, as in finite state controllers; indexical features, whose values are a function of the state and a number of internal registers that can be loaded with objects; and modules that wrap up policies and sketches and allow them to call each other by passing parameters. In addition, unlike general policies that select state transitions rather than ground actions, the new language allows for the selection of such actions. The expressive power of the resulting language for policies and sketches is illustrated through a number of examples.

==> bib/README <==
Before adding entries to any of the files in the bibliography
repository, please carefully read the instructions at the beginning
of literatur.bib!

If you add conference papers of conferences which are likely to be
cited multiple times, please add cross reference entries in both
crossref.bib and crossref-short.bib. See also the instructions at
the beginning of these files.

Usage: \bibliography{abbrv,literatur,crossref}


==> chapters/acknowledgements.tex <==

\section*{Acknowledgments}

The research of H.\ Geffner has been supported by the Alexander von Humboldt Foundation with funds from
the Federal Ministry for Education and Research. The research  has also  received funding from
the European Research Council (ERC), Grant agreement No.\ No 885107, and Project TAILOR,
Grant agreement No.\ 952215,  under EU Horizon 2020 research and innovation programme,
the Excellence Strategy of the Federal Government and the NRW L\"{a}nder, and
the Knut and Alice Wallenberg (KAW) Foundation under the WASP program.
%% This work was partially supported by an ERC Advanced Grant (grant
% agreement no.\ 885107), by project TAILOR, funded by EU Horizon 2020
% (grant agreement no.\ 952215), and by the Wallenberg AI,
% Autonomous Systems and Software Program (WASP)
% funded by the Knut and Alice Wallenberg Foundation.
% Hector Geffner is a Wallenberg Guest Professor at
% Link{\"o}ping University, Sweden.
% Acknowledge NAISS and SNIC
% https://www.naiss.se/policies/acknowledge/acknowledge-naiss-snic/
% https://www.nsc.liu.se/
% \alert{** Which computations? **}
% The computations were enabled by resources provided by the
Resources were also provided by the National Academic Infrastructure for Supercomputing in Sweden (NAISS)
and the Swedish National Infrastructure for Computing (SNIC) at
the National Supercomputer Centre at Link{\"o}ping University partially funded by the
Swedish Research Council through grant agreements no.\ 2022-06725 and no.\ 2018-05973.



